Self-Supervised Multi-Object Tracking For Autonomous Driving From Consistency Across Timescales

Self-supervised multi-object trackers have tremendous potential as they enable learning from raw domain-specific data. However, their re-identification accuracy still falls short compared to their supervised counterparts. We hypothesize that this drawback results from formulating self-supervised objectives that are limited to single frames or frame pairs. Such formulations do not capture sufficient visual appearance variations to facilitate learning consistent re-identification features for autonomous driving when the frame rate is low or object dynamics are high. In this work, we propose a training objective that enables self-supervised learning of re-identification features from multiple sequential frames by enforcing consistent association scores across short and long timescales. We perform extensive evaluations demonstrating that re-identification features trained from longer sequences significantly reduce ID switches on standard autonomous driving datasets compared to existing self-supervised learning methods, which are limited to training on frame pairs. Using our proposed SubCo loss function, we set the new state-of-the-art among self-supervised methods and even perform on par with fully supervised learning methods.

==> figures/demo_2/figure.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[trim=0 0 0 0,clip,width=\textwidth]{figures/demo_2/frame0_trackid6.jpg}
        \caption{Reference frame}
        \label{fig:demo1_ref}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[trim=0 0 0 0,clip,width=\textwidth]{figures/demo_2/frame1_trackid6_use-bbox-iou.jpg}
        \caption{Bbox IoU}
        \label{fig:demo1_bbox_only}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[trim=0 0 0 0,clip,width=\textwidth]{figures/demo_2/frame1_trackid6_use-reid_swav.jpg}
        \caption{MoCo v2 ReID}
        \label{fig:demo1_moco}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[trim=0 0 0 0,clip,width=\textwidth]{figures/demo_2/frame1_trackid6_use-reid.jpg}
        \caption{Ours ReID}
        \label{fig:demo1_ours}
    \end{subfigure}
    
    \caption{Qualitative \gls{mot} results on \gls{bdd} comparing varying association methods for sequence \textit{b1c66a42-6f7d68ca}.}
    \label{fig:qualitative_example_mot}
\end{figure*}

==> sections/61_supp_assigner.tex <==
\begin{table*}[]
\scriptsize
\centering
\caption{Assignment error of various approximate bipartite matching methods compared to optimal cost assignment by Hungarian algorithm~\cite{hungarianmethod}. Results are calculated for 1000 runs on random cost matrices sampled from the interval $[0, 1]$, and runtimes are reported as average. $h$ represents the threshold for assigning to the insertion/deletion class.}
\label{tab:supp_matcher_testbed}
\begin{tabular}{cccccccccc} \toprule
Method & $[0, 1]^{n \times m }$& \multicolumn{2}{c}{h = 0.0} & \multicolumn{2}{c}{h = 0.25} & \multicolumn{2}{c}{h = 0.5} & \cite{brun2022lsape} [ms] & HM~\cite{hungarianmethod}[ms] \\ 
 & & $\mu$ & $\sigma^2$ & $\mu$ & $\sigma^2$ & $\mu$ & $\sigma^2$  &  &  \\ \midrule
\multirow{4}{*}{\cite{brun2022lsape}} & 10 $\times$ 10 & 33.11 & 43.08 & 21.59 & 46.32 & 11.68 & 26.19 & 0.70 & 0.08 \\
 & 10 $\times$ 20 & 46.12 & 63.72 & 27.02 & 65.41 & 25.26 & 65.89 & 0.41 & 0.08 \\
 & 20 $\times$ 20 & 34.32 & 21.60 & 33.12 & 23.34 & 14.00 & 24.77 & 1.08 & 0.15 \\
 & 20 $\times$ 30 & 45.09 & 28.44 & 35.20 & 28.35 & 35.52 & 31.32 & 0.61 & 0.14 \\ \midrule
\multirow{4}{*}{BPMN} & 10 $\times$ 10 & 11.13 & 13.25 & 10.09 & 13.01 & 9.32 & 12.94 & 0.34 & 0.08 \\
 & 10 $\times$ 20 & 10.92 & 13.03 & 10.81 & 12.73 & 11.78 & 12.18 & 0.34 & 0.08 \\
 & 20 $\times$ 20 & 11.35 & 10.12 & 11.08 & 9.78 & 11.43 & 10.09 & 0.37 & 0.15 \\
 & 20 $\times$ 30 & 8.81 & 10.13 & 8.18 & 10.75 & 7.30 & 10.67 & 0.58 & 0.14 \\
 \bottomrule
\end{tabular}
\end{table*}



==> sections/62_supp_degenerate_cases.tex <==
\subsection{Discussion degenerate cases}

The self-supervised learning task proposed in the main paper can be ill-defined for specific configurations.
One such scenario is given when no two object detections in a sequence correspond to each other. In this configuration, all tracks are deleted, which leaves no associations to compute a loss value for.
Such a scenario is possible, e.g. with large camera rotation between frames, such that the  field of views of the initial and final camera perspectives have zero overlaps. For the datasets used in our paper, \ie \gls{mot17} and \gls{bdd}, we, therefore, performed an overlap analysis of the annotated subsets, which is depicted in \figref{}.
For this analysis, we computed the histogram of track lengths for the entire dataset and each split separately on the left side. 
The right side shows the union ratios of track IDs between all frames for variable sequence lengths.
We find that the dataset does not contain the potential for such degenerate cases.
Therefore, such degenerate cases would only arise when the object detector outputs imperfect predictions. In such cases, we skip parameter updates for this sample.

\input{tables/supp_dataset_track_stats}

We would like to point out, that most self-supervised pre-training task suffers from some sort of edge cases, that results in degenerate loss computation. 
For example, image augmentations like cropping used in almost all contrastive approaches could remove the principal object from the image, if it is located at a border region and not occupying sufficient areas of the image.

In our case, we could filter out such scenarios, where a pre-trained tracker loses all tracks within the length of a sample sequence. Another scenario would be to pre-train our method on examples, where we can ensure that all tracks survive the sample length. Then, this self-supervised tracker is trained on a curated subset of the training data to perform the filtering. 

==> tables/supp_dataset_track_stats.tex <==
\begin{table*}[]
\scriptsize
\centering
\caption{Dataset track statistics for the \gls{bdd} and \gls{mot17} annotations. Overlap is computed for a sequence length of $N=4$ and $N=8$ respectively.}
\label{tab:dataset_stats}
\begin{tabular}{c|cccc|cccc|cccc|cccc} \toprule
 & \multicolumn{4}{c|}{instances per frame} & \multicolumn{4}{c|}{Overlap (N=4) [\%]} & \multicolumn{4}{c|}{Overlap (N=8)[\%]} & \multicolumn{4}{c}{Track length} \\ 
 & q=5\% & q=95\% & mean & std & q=5\% & q=95\% & mean & std & q=5\% & q=95\% & mean & std & q=5\% & q=95\% & mean & std \\ \midrule
BDD100k train & 2 & 57 & 9.98 & 5.84 & 44.4 & 100.0 & 77.7 & 18.6 & 25.0 & 100.0 & 65.7 & 22.4 & 2 & 203 & 18.54 & 26.21 \\
BDD100k val & 2 & 49 & 11.25 & 6.85 & 45.5 & 100.0 & 77.1 & 18.2 & 27.3 & 100.0 & 65.1 & 21.6 & 1 & 203 & 17.94 & 25.80 \\ \midrule
MOT17 half-train & 7 & 49 & 21.92 & 13.44 & 81.8 & 100.0 & 96.2 & 6.5 & 72.7 & 100.0 & 93.2 & 9.1 & 7 & 526 & 162.69 & 157.92 \\
MOT17 train & 6 & 52 & 21.12 & 14.34 & 81.8 & 100.0 & 95.9 & 7.2 & 71.4 & 100.0 & 92.6 & 10.1 & 7 & 1050 & 205.29 & 256.19 \\
MOT17 half-val & 5 & 52 & 20.32 & 15.15 & 81.8 & 100.0 & 95.6 & 7.9 & 69.8 & 100.0 & 92.0 & 11.0 & 8 & 524 & 158.49 & 157.13 \\ \bottomrule
\end{tabular}
\end{table*}
